A Nitrogen-rich AGN Powering a Large Ionizing Bubble at z=8.63

We report the detection of Ly${\alpha}$ in CANUCS-LRD-z8.6, a recently discovered AGN at z = 8.63 by Tripodi et al. (2024), in new NIRSpec/MSA G140H/F070LP observations. We detect broad Ly${\alpha}$ emission (FWHM $= 1540 \pm 260$ km/s) near the systemic velocity, which suggests a large ionizing bubble considering that the universe is almost fully neutral at the redshift. Through Ly${\alpha}$ line-shape modeling assuming a Stromgren sphere, we find a large bubble radius, $R_b = 1.5^{+0.3}_{-0.2}$ pMpc, and a moderately high Ly${\alpha}$ escape fraction, $f_{esc} = 11 \pm 3$ %. The intrinsic line width is inferred to be broad ($2200 \pm 280$ km/s), likely originating in the broad-line region. Existing data indicate that CANUCS-LRD-z8.6 is within a mild overdensity, $\delta = 1.8^{+3.0}_{-0.6}$, suggesting that other galaxies in its proximity might have contributed to the formation of the bubble. The high N IV]${\lambda}$1488 / C IV${\lambda}$1548 and N IV]${\lambda}$1488 / O III]${\lambda}$1661 line ratios measured in existing NIRSpec/PRISM data indicate nitrogen enrichment in this metal-poor, low-luminosity AGN. The spectroscopic features are overall similar to other nitrogen-rich galaxies discovered in the literature, such as GN-z11 and GHZ2/GLASSz12. This suggests that CANUCS-LRD-z8.6 may represent one of the evolutionary phases of those nitrogen-rich galaxies.

==> table_phys.tex <==
\begin{deluxetable*}{ccc}
    \tabletypesize{\footnotesize}
    \tablecolumns{3}
    \tablewidth{0pt}
    \tablecaption{
    Physical properties of \id}
    \tablehead{
    \colhead{Property} & \colhead{Unit} & \colhead{Measurement}\\
\colhead{} & \colhead{} & \colhead{}
}
    \startdata
R.A. & degree & $1.773909e+02$\\
Decl. & degree & $2.234977e+01$\\
$z$ &  & $8.6319\pm0.0005$\\
$\mu$ &  & $1.85_{-0.02}^{+0.02}$\\
$M_*$ & $\log M_\odot$ & $8.8_{-0.0}^{+0.0}$\\
$A_{V, \mathrm{SED}}$ & mag & $0.2_{-0.0}^{+0.0}$\\
$M_\mathrm{UV}$ & mag & $-19.30_{-0.03}^{+0.04}$\\
$\mathrm{SFR_{UV}}$ & $\log M_\odot {\rm yr^{-1}}$ & $0.79_{-0.03}^{+0.03}$\\
$\mathrm{SFR_{100Myr}}$ & $\log M_\odot {\rm yr^{-1}}$ & $0.80_{-0.03}^{+0.02}$\\
$\mathrm{SFR_{H\beta}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.18_{-0.05}^{+0.05}$\\
$\beta_{\mathrm{UV, SED}}$ &  & $-1.5$\\
$\beta_{\mathrm{UV, photometry}}$ &  & $-2.3$\\
$A_{V,\mathrm{nebular}}$ & mag & $0.0$\\
$12 + \mathrm{\log (O/H)}$ &  & $7.08_{-0.06}^{+0.05}$\\
% $R_e$ & kpc & $0.11_{-0.01}^{+0.01}$\\
\enddata
\tablecomments{
    Measurements are corrected for magnification using $\mu=1.85$. $\mathrm{SFR_{H\beta}}$ is derived using the narrow \hb\ line flux.
    }\label{tab:phys}
    \end{deluxetable*}
